Event-Centric Query Expansion in Web Search

In search engines, query expansion (QE) is a crucial technique to improve search experience. Previous studies often rely on long-term search log mining, which leads to slow updates and is sub-optimal for time-sensitive news searches. In this work, we present Event-Centric Query Expansion (EQE), a novel QE system that addresses these issues by mining the best expansion from a significant amount of potential events rapidly and accurately. This system consists of four stages, i.e., event collection, event reformulation, semantic retrieval and online ranking. Specifically, we first collect and filter news headlines from websites. Then we propose a generation model that incorporates contrastive learning and prompt-tuning techniques to reformulate these headlines to concise candidates. Additionally, we fine-tune a dual-tower semantic model to function as an encoder for event retrieval and explore a two-stage contrastive training approach to enhance the accuracy of event retrieval. Finally, we rank the retrieved events and select the optimal one as QE, which is then used to improve the retrieval of event-related documents. Through offline analysis and online A/B testing, we observe that the EQE system significantly improves many metrics compared to the baseline. The system has been deployed in Tencent QQ Browser Search and served hundreds of millions of users. The dataset and baseline codes are available at https://open-event-hub.github.io/eqe .

==> backup.tex <==
\subsection{Event Collection}

%伟杰
% 事件扩展候选挖掘是整个系统最基础的一部分， 要求能实时、全面发现全网的热点事件内容。在这个系统中， 事件候选可以分成 基于doc的候选挖掘和 基于query的候选挖掘
The most important component of QEE is "Event Collection", which is utilized to thoroughly gather hot events from all across the network in real-time. Both document-based and query-based approaches can be used.

% Event expansion candidate mining is the most basic part of the whole system, which requires real-time and comprehensive discovery of hot events in the whole network. 
% In this system, event candidates can be divided into doc-based candidate mining and query-based candidate mining.

% 1、 基于doc 的候选挖掘
\subsubsection{Doc-based Method}

% 在QQ浏览器搜索中，每天有海量的新增conetent。在xxx 系统中， 为便于后续的事件挖掘和正规化， 需要从海量的内容中识别事件内容。
%  文章的标题是一篇文章最核心的部分，与此相反， 正文内容充斥着大量的噪声信息。我们收集了QQ浏览器近半年的新闻标题， 对标题进行事件判别。
% 首先，在xxx中， 我们首先根据网页的发布时间、页面类型、质量、账号和site 等特征， 做粗略过滤。 随着自媒替内容越来越多样化，这些基于启发式的规则过滤是不够的.	根据统计，语法不规则、成本缺失 、事件触发词缺失、多事件等问题， 给后续的事件正规划 带来挑战。 所以， 我们是会用工具LTP 提取标题中的事件触发词， 对缺事件和多事件（事件触发词>2)的内容过滤。 然后， 我们构建了一个语义判别模型，用于从大量的新闻标题中识别出事件内容。
% 经过专家标注获得大量的有监督样本，将样本喂给PLM模型BERT， 就得到了新闻标题的事件概率，Given a news title T，T={t1, t2,，，， tn}， 表示输入的title序列，。 通过将其喂给预训练模型， 就能获得其最终的事件概率， 通过控制概率阈值为xx， 我们获得了事件判别的准确率达到95%。

% In QQ Browser search, there are a large number of new conetent every day. In the xxx system, in order to facilitate the subsequent event mining and normalization, it is necessary to identify the event content from the massive content.
% The title of an article is the core of an article, on the contrary, the text is full of a lot of noise information.

% We collected QQ Browser's news headlines for nearly half a year to judge the events of the headlines.
% First of all, in xxx, we first do rough filtering according to the release time, page type, quality, account and site of the web page. As the content of self-media becomes more and more diverse, these heuristic rule-based filtering is not enough. According to statistics, irregular grammar, lack of cost, lack of event triggers, multiple events and other problems bring challenges to the follow-up event planning. Therefore, we will use the tool LTP to extract event triggers in the title and filter the content of missing events and multiple events (event triggers > 2). Then, we build a semantic discrimination model to identify event content from a large number of news headlines.
% After expert tagging, a large number of supervised samples are obtained, and the samples are fed to the PLM model BERT, and the event probability of the news headline is obtained, Given a news title TMagi T = {T1, T2 tn}, which represents the input title sequence. By feeding it to the pre-training model, the final event probability can be obtained. By controlling the probability threshold to xx, the accuracy of event discrimination is up to 95%.
Everyday, a vast number of fresh documents are uploaded to the Internet. Therefore, the initial step of "Event Collecting" is to find events among these huge contents. To do this, we utilize a two-step procedure comprised of \textit{rough filtering} and \textit{semantic filtering}.

\textit{\textbf{Rough filtering.}} In general, an article's headline is the most important element, whereas the body contains a great deal of irrelevant material.
After using basic feature filters such as publication time, page type, site type, etc., we gathered approximately 50 million news article headlines over the duration of recent six months.
As seen in Table 1, the headlines generated by these heuristic rules include irregular syntax, missing event components, numerous events, etc., posing a barrier for the subsequent event normalization.
So further we use LTP~\citep{che-etal-2021-n} to extract event triggers from headlines, and drop headlines missing event elements or with multiple events (the number of triggers is greater than 2). 

\textit{\textbf{Semantic filtering.}} Then, an event detection model is constructed to find further event possibilities. With two experts annotating, about 200,000 samples are supervised-labeled. We finetune a RoBERTa as the event detection model and infer the rest data to derive event probabilities of headlines. By filtering event probabilities with a predefined threshold, we are able to produce 95\% correct event headlines.

% Then, we build a semantic discrimination model to identify event content from a large number of news headlines.
% After expert tagging, a large number of supervised samples are obtained, and the samples are fed to the PLM model BERT, and the event probability of the news headline is obtained, Given a news title TMagi T = {T1, T2 tn}, which represents the input title sequence. By feeding it to the pre-training model, the final event probability can be obtained. By controlling the probability threshold to xx, the accuracy of event discrimination is up to 95%.

% \begin{equation}
% \begin{aligned}
% c= PLM(Title) 
% y = softmax(W c+b)
% \end{aligned}
% \end{equation}

\subsubsection{Query-based Method}

% 对于突发事件，搜索频次序列存在明显的突变趋势. 我们基于峰值探测算法来挖掘热点query。首先， 统计一段事件内的搜索qv，按照相同的时间窗口将频次 构造成序列。 为了避免频次在天级内的周期性变化， 频次选择是至关重要的 我们选择每天相同时间段的qv 构造序列。
% Q=（qv1、qv2、qv3.。。。qvn)ff
% 然后 按照公式2、3 计算对应的cv 系数。 通过控制阈值 对大于xx的query作为事件候选。
% \textit{Query sequence analysis.} For emergencies, the search frequency sequence has an obvious sudden change trend. We mine hot query based on peak detection algorithm. First of all, the search qv within a period of events is counted, and the frequency is constructed into a sequence according to the same time window. In order to avoid the periodic change of the frequency within the sky level, the frequency selection is very important. We choose the qv construction sequence at the same time every day.set Query freqency sequence $Q=\{qv_1, qv_2..., qv_n\}$，

% Then the corresponding cv coefficients are calculated according to formulas 2 and 3. The query larger than xx is selected as the event candidate by controlling the threshold.


\textit{Query sequence analysis.} For breaking news, there is a typical bursting trend in query frequency sequences. 
To identify such burst signals in queries, we use a peak detection algorithm.
Given a search query Q, its search frequency is divided into sequences $Q=\{qv_1, qv_2..., qv_n\}$， according to a fixed time window. 
To avoid periodic changes in frequency during the day, the frequencies are usually from the same window in the day.

As shown in Eqs. 1 to 3, the burst factor $QCV$ of the query can be calculated by calculating the average and weighted variances of the frequency sequences. Usually, the $QCV$ is higher than the normal query for an event query that is occurring. To obtain a burst event query, we set a hyper-parameter (we set $\alpha = 0.94 \beta = 0.001 QCV > xx$).

% \begin{equation}
\begin{gather}
Avg = {\frac{1}{N} }{\sum_i^N(qv_i)}\\
Std = \sqrt{{\frac{1}{N} }{\sum_i^N{ \alpha \cdot (qv_i - Avg)^2 }}}\\
QCV =  \frac{Std}{Avg+ \beta } 
\end{gather}
% \end{equation}
   
% \begin{figure}[ht]
%     \vspace{-1em}
%     \centering
%     \setlength{\abovecaptionskip}{0cm}  %调整图片标题与图距离
%     % \setlength{\belowcaptionskip}{-0.8cm} %调整图片标题与下文距离
%     \includegraphics[scale=0.]{figures/qcv.png}
%     \caption{qcv}
%     \label{fig:ugc_data}
%     \vspace{-0.5em}
% \end{figure}


% 	b) 基于图的事件识别
% 时效性query 呈现典型的聚类效果。 通过构建query-doc的点击图（参考）， 通过迭代能聚类出query和query的相关性。为保证挖掘结果的时效性， 仅保留发布时间在最近的，且新闻类型结果的点击数据， 这类query通常指向正在发生的事件。
% 搜索query 存在比较典型的长尾特点，点击图聚类出的query 会存在大量的噪音信息。在实时聚类出的所有query簇中， 根据簇中query数量、query 搜索频次过滤掉长尾query。最终提取簇类的高频query， 作为候选事件。

\textit{Query graph analysis.} In general, time-sensitive queries exhibit typical clustering effects. To capture the clustering signals of queries, we devise a Query-Document click graph $\mathcal{G}$ based on the click propagation algorithm. To minimize the noise stemming from non-time-sensitive queries, we only consider click pairs from news pages within a 3-day period. The Query and Document representations are iteratively updated according to Equations xx and xx, respectively.
\begin{gather}
    Q_{i}^{\left ( n \right ) } = \frac{1}{\left \|  {\textstyle \sum_{j}^{\left | Doc \right | }C_{i,j}\cdot D_{j}^{\left ( n- 1 \right ) } }  \right \|_2  } \sum_{j = 1}^{\left | Doc \right | } C_{i,j}\cdot D_{j}^{\left ( n- 1 \right ) }
    \\
    D_{j}^{\left ( n \right ) } = \frac{1}{\left \|  {\textstyle \sum_{i = 1}^{\left | Query \right | }C_{i,j}\cdot Q_{i}^{\left ( n \right ) } }  \right \|_2  } \sum_{i = 1}^{\left | Query \right | } C_{i,j}\cdot Q_{i}^{\left ( n \right ) }
\end{gather}
% where Q denotes the representation of Query and Di denotes the representation of Document.
where $Q_{i}^{\left ( n \right ) } $ is the representation of query $q_i$ at the $n$-th iteration.

Unlike the original click propagation algorithm, after the n-th iteration, we only use the Query representation to obtain the Query clusters. However, the sparsity problem also persists for time-sensitive queries. To mitigate this risk, we filter out the low-frequency queries from the clusters and eventually select the high-frequency queries 
% from the clusters 
as event candidates.



\textbf{Online Evaluation.} 
We implement online ab testing to study the online performance of the system.

we deploy the QEE framework to the QQ Browser search online system to illustrate its actual effect. The following metrics are considered:(i)  (converage), (ii) click-through rate (CTR), (iii) click percentage. As mentioned above, in order to improve user search experience, we utilize QE for downstream tasks (search recalls, and sorting). In the experiment, we conducted a 7-day AB experiment and obtained 1\% of the real traffic online. For comparison, we use the strong baseline described in 4.1 as the control group. As shown in Table xx, we observed expansion coverage, CTR, dot rate and other indicators of all kinds of business cards during the experimental period. Among them, card coverage increases xx, CTR improves xxx, and a little bit increases xx. Through experimental indicators, it can be proved that QE model can significantly improve business effect and user experience.

\subsection{Performance of the data collection scheme.} 
In fact, it is difficult to find all the events happening completely, so this problem has been approximated - through the events from breaking news list, while users always pay more attention to these events and hope to get complete relevant information more quickly. We collected the breaking news list of the whole Chinese website for seven consecutive days, including Baidu, Weibo, etc., as well as the logs of QEE and baseline data collection modules. Two annotation experts employed assisted in the evaluation: 1)aggregate these events from different sources to find the earliest time they appeared; 2)find the occurrence time of the the event (the time when the first report emerged on the network); 3)detect the earliest time of events in QEE and baseline by keyword search.

Figure 7 shows the average coverage of QEE, baseline, and breaking news list at different time points after the event occurred. QEE discovered the incident in time with a huge advantage of xxmin.




\subsection{Performance of Generation Model.} 

In this section, we evaluate the performance of the proposed generation model by computing automated metrics and human evaluation metrics. We disclose our test dataset, which is called Title2EventPhrase, and introduce its production details in Appendix~\ref{sec:Title2EventPhrase_dataset} and \ref{sec:Title2EventPhrase_ana}. We conduct ablation experiments to measure the effect of the prompt module and the contrastive learning module. Furthermore, to verify the universality of the two modules, we used BART and mT5 as the backbone networks, respectively. 

a). Automated evaluation. Automated metrics are compared using the ROUGE, BLEU and BERTScore metrics on the labeled test dataset. As shown in Table~\ref{tab:automated}, our proposed components significantly improved the generation performance.

\begin{table}[t]
\small
\begin{tabular}{l|lll}
\hline
model         & Rouge-L & BLEU & BERTScore \\ \hline
BART(vanilla) &   0.8405    &   0.7706    &  0.9271 \\ 
BART+CL    &    0.8416   &   0.7733  & 0.9282 \\ 
BART+PG    &  0.8473  &  0.7792  & 0.9299 \\ 
BART+CL+PG    & 0.8495  & 0.7840  &  0.9319 \\ \hline
mT5(vanilla)  &   0.8464    &   0.7789    &  0.9302   \\  
mT5+CL  &  0.8503     &   0.7845   &   0.9321    \\ 
mT5+PG  &  0.8522     &  0.7868    &  0.9327 \\ 
mT5+CL+PG   &  0.8545      &  0.7907  & 0.9341 \\ \hline
\end{tabular}
\caption{Automated evaluation of ablation experiments. CL and PG are abbreviations for contrastive learning and prompt guidance respectively}
\label{tab:automated}
\end{table}

b). Human evaluation. Considering the fluency, accuracy and consistency of the generated content, we set a scoring standard of levels from 1 to 5 for the model generation results, of which 1 is the worst and 5 is the best. See the appendix for the meaning of the indicators corresponding to each score. After scoring $n$ pieces of data by two professional annotators, Table~\ref{tab:human-eval} shows the results. The proposed generation model has higher scores in terms of grammatical norms and generative loyalty.


\subsection{Online Ranking}
%调换顺序、词汇统一，时效性
% 在xxx中，仅仅依靠query检索的语义相关性是不够的. 事件扩展将结合相关性、热度、时效性等多维度信息， 决定最终选择那一个query扩展.受限于线上服务性能要求，  我们采用了一个经典的轻量级排序模型GBDT。 同时这个模型对线上特征的解释是非常友好。
% 特征工程。 我们使用了三类特征来构建模型。
% 1） query侧特征， 我们构建了例如query频次、query本身的突发语义、来自搜索query理解的通用信号， 比如意图分类、实体信息等
% 2） 事件特征：语义检索打分。 BM25、核心词命中等是重要的相关性特征。 同时，在xx系统中， 正规化事件被用于在线聚类模型， 聚类簇产出的信息比如簇大小、簇聚合频次等是重要的需求强度信号
% 3） doc侧特征：比如搜索召回doc 的时效性、相关性分布等等
% 样本收集：首先我们部署了一个1%流量的在线ab实验用于收集样本。在整个搜索需求中， 时效性的占比较少， 通常为<10%. 首先我们用一个先验的query语义模型， 粗略的过滤掉大量的非时效性query。从过滤后的query、event召回结果中，富集大量的线上样本。 经过大量的专家标注获得约10w样本。经过GBDT模型排序，我们最终选取排序后的top1结果作为query扩展。对query 扩展， 我们进行了系统性效果评估：准确率：95% 召回率:92%. 

In QEE, event expansion will combine multiple pieces of information, such as relevance, heat, and timeliness, to determine which query expansion to choose. It is no longer enough to rely solely on the semantic relevance of query retrieval due to the limited performance requirements of online services, so we use the classic lightweight sorting model GBDT. This model is very friendly to the interpretation of online features.
%Feature engineering. 

We used three types of features to build the model.

1) query side features, such as query frequency, burst semantics of query itself(存在疑问), general signals from query understanding, such as intention classification, entity information, etc.

2) event characteristics: semantic retrieval scoring. BM25 and medium core words are important correlation features. At the same time, in the xx system, normalization events are used in the online clustering model, and the information produced by clusters, such as cluster size and cluster aggregation frequency, is an important demand intensity signal.

3) doc side features, such as timeliness and correlation distribution of search recall doc, etc.
Sample collection: first, we deploy an online ab experiment with 1\% traffic to collect samples. In the whole search demand, timeliness accounts for less, usually < 10\%. First of all, we use a priori query semantic model to roughly filter out a large number of non-timed query. A large number of online samples were enriched from the filtered query and event recall results. After a large number of expert labeling, about 10w samples are obtained. After sorting by the GBDT model, we finally select the sorted top1 result as the query expansion. For query expansion, we evaluated the systematic effect: accuracy: 95\% recall rate: 92\%.
